Learning to Recover Spectral Reflectance from RGB Images

This paper tackles spectral reflectance recovery (SRR) from RGB images. Since capturing ground-truth spectral reflectance and camera spectral sensitivity are challenging and costly, most existing approaches are trained on synthetic images and utilize the same parameters for all unseen testing images, which are suboptimal especially when the trained models are tested on real images because they never exploit the internal information of the testing images. To address this issue, we adopt a self-supervised meta-auxiliary learning (MAXL) strategy that fine-tunes the well-trained network parameters with each testing image to combine external with internal information. To the best of our knowledge, this is the first work that successfully adapts the MAXL strategy to this problem. Instead of relying on naive end-to-end training, we also propose a novel architecture that integrates the physical relationship between the spectral reflectance and the corresponding RGB images into the network based on our mathematical analysis. Besides, since the spectral reflectance of a scene is independent to its illumination while the corresponding RGB images are not, we recover the spectral reflectance of a scene from its RGB images captured under multiple illuminations to further reduce the unknown. Qualitative and quantitative evaluations demonstrate the effectiveness of our proposed network and of the MAXL. Our code and data are available at https://github.com/Dong-Huo/SRR-MAXL.

==> 7_biography.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{portrait/Dong.jpg}}]{Dong Huo}
received the B.Eng. degree in Software Engineering from the Harbin Institute of Technology, Harbin, China, in 2018. He is currently persuing his Ph.D. in the Department of Computing Science, University of Alberta, Canada. His research interests include computer vision, image processing, deep learning, and machine learning, with a focus on image restoration, meta-learning and generative models.
\end{IEEEbiography}


\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{portrait/Jian.jpeg}}]{Jian Wang} received the B.Eng. degree from the Xi’an Jiao Tong University,
Xi’an, China, in 2009, the M.Sc. degree from the University of Science and Technology of China, Hefei, China, in 2013, and the Ph.D. degree from the Electrical and Computer Engineering department, Carnegie Mellon University, Pittsburgh, USA, in 2018. He is currently Senior Research Scientist in Snap Inc, New York, USA. His research interests include computer vision, computational imaging and computational photography.
\end{IEEEbiography}




\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{portrait/yiming.jpeg}}]{Yiming Qian} received the B.Sc. degree from the University of Science and Technology of China,
Hefei, China, in 2012, the M.Sc. degree from the Memorial University of Newfoundland, St. John’s, Canada, in 2014, and the Ph.D. degree from the Department of Computing Science, University of Alberta, Edmonton, Canada, in 2019. He is currently an Assistant Professor with the University of Manitoba, Canada. His research interests include computer vision and computer graphics, while he recently focuses on 3D modeling.
\end{IEEEbiography}


\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{portrait/Yee-Hong.jpg}}]{Yee-Hong Yang}
(Senior Member, IEEE) received the B.Sc. degree (Hons.) from The University of Hong Kong, the M.Sc. degree from Simon Fraser University, and the Ph.D. degree from the University of Pittsburgh. He was a Faculty Member of the Department of Computer Science, University of Saskatchewan, from 1983 to 2001, and served as the Graduate Chair from 1999 to 2001. While there, in addition to department level committees, he also served on many college and university level committees. Since July 2001, he has been a Professor with the Department of Computing Science, University of Alberta, where he served as the Associate Chair (Graduate Studies) from 2003 to 2005. His research interests cover a wide range of topics from computer graphics to computer vision, which include physically based animation of Newtonian and non-Newtonian fluids, texture analysis and synthesis, human body motion analysis and synthesis, computational photography, stereo and multiple view computer vision, and underwater imaging. He has published over 160 papers in international journals and conference proceedings in the areas of computer vision and graphics. He serves on the Editorial Board of the journal Pattern Recognition. In addition to serving as a reviewer to numerous international journals, conferences, and funding agencies, he has served on the program committees of many national and international conferences. In 2007, he was invited to serve on the expert review panel to evaluate computer science research in Finland.
\end{IEEEbiography}

==> tables/ablation_1.tex <==
\begin{table}[t]
\centering
\renewcommand\arraystretch{1.5}
\setlength\tabcolsep{5pt}
\caption{Ablation studies of network components.}
\begin{tabular}{lccc}
\toprule
Methods                       & MAE$\downarrow$   & RMSE$\downarrow$  & SAS$\downarrow$     \\ 
\midrule
Ours (pre-trained)            & \textbf{0.0625} & \textbf{0.0828} & \textbf{0.0748} \\ 
w/o pyramid                   & 0.1277      &  0.1585     & 0.1432    \\ 
w/o FUSE                   & 0.0676      & 0.0887      & 0.0803      \\ 
w/ zero $m^i$ in FUSE       & 0.0711      &  0.0922     & 0.0830    \\               
w/o $\hat{\mathbf{R}}_{\hat{\boldsymbol{\mathcal{H}}}}^i$                 & 0.0669      & 0.0876      & 0.0798 \\
w/o $\hat{\omega}^i$       & 0.0691      & 0.0909      & 0.0824      \\ 
w/ ground truth CSSs    & \textbf{0.0621}     & \textbf{0.0824}     & \textbf{0.0744}      \\ 
w/o spectral-attention        & 0.0730 & 0.0958 & 0.0894     \\ 
w/o auxiliary task            & 0.0674      & 0.0888      & 0.0796     \\ 
\bottomrule
\end{tabular}
\label{tab:ablation_1}
\end{table}
% \jian{also label the 2nd best}


==> tables/ablation_2.tex <==
\begin{table}[t]
\centering
\renewcommand\arraystretch{1.5}
\setlength\tabcolsep{5pt}
\caption{Ablation studies of learning strategies.}
\begin{tabular}{lccc}
\toprule
Methods                       & MAE$\downarrow$   & RMSE$\downarrow$  & SAS$\downarrow$     \\ 
\midrule
Ours (pre-trained)            & 0.0625 & 0.0828 & 0.0748 \\ 
w/ meta-auxiliary training    & 0.0611     & 0.0814   & 0.0739   \\ 
w/ test-time adaptation   & 0.0624 & 0.0827 & 0.0745  \\ 
w/ MAXL   & \textbf{0.0607} & \textbf{0.0809} & \textbf{0.0734} \\ \bottomrule
\end{tabular}
\label{tab:ablation_2}
\end{table}
